GooAQ: Open Question Answering with Diverse Answer Types

While day-to-day questions come with a variety of answer types, the current question-answering (QA) literature has failed to adequately address the answer diversity of questions. To this end, we present GooAQ, a large-scale dataset with a variety of answer types. This dataset contains over 5 million questions and 3 million answers collected from Google. GooAQ questions are collected semi-automatically from the Google search engine using its autocomplete feature. This results in naturalistic questions of practical interest that are nonetheless short and expressed using simple language. GooAQ answers are mined from Google's responses to our collected questions, specifically from the answer boxes in the search results. This yields a rich space of answer types, containing both textual answers (short and long) as well as more structured ones such as collections. We benchmarkT5 models on GooAQ and observe that: (a) in line with recent work, LM's strong performance on GooAQ's short-answer questions heavily benefit from annotated data; however, (b) their quality in generating coherent and accurate responses for questions requiring long responses (such as 'how' and 'why' questions) is less reliant on observing annotated data and mainly supported by their pre-training. We release GooAQ to facilitate further research on improving QA with diverse response types.

==> UNUSED/conclusion-OLD.tex <==
\section{Conclusion}
We studied open question-answering under diverse response types. 
For this purpose, we collected \name{}, a very large collection of QA pairs mined from Google, with a variety of (short and long) answer types, all of which are collected using a unified, coherent process, enabling a cross-type comparison. The questions are collected from the auto-complete system, which likely reflects a \emph{natural} distribution of questions asked by users. 
% The answers are mined from Google answer boxes. 

We benchmarked two variants of a state-of-the-art self-contained text generation model (T5, with no retrieval) on the three different sub-tasks of \name{} (short, snippet, and collection), and using both automatic and human evaluations. Our analysis brings out the distinct behavior of LMs on long and short response questions. For example, while short response models benefit heavily from more labeled data, the surprisingly strong performance of long response models is driven mostly by their pre-training. We also demonstrate that \name{} is a valuable model training resource, via high zero-shot performance on an extrinsic task, ELI5.

We hope our analysis and the released data will benefit the understanding of and further development of QA systems for dealing with diverse response types. 



==> UNUSED/discussion-OLD.tex <==
\section{Discussion}
\label{sec:discussion}
\hanna{Maybe merge Discussion and conclusion, rename this section: Conclusion and Discussions 
Then we can organize this section as this:
1. Conclusions: copy the first two parags of the conlusion 
2. Scope of our conclusions: 
merge "knowledge leakage and scope of our conclusion paragraphs"
3. Are we mimicking google?
4. Future uses of Guac: merge "other uses of GooAQ + replicating human eval + there is still a lot of room to improve + we can use Quac for question generation" }
\paragraph{Knowledge leakage in the evaluation.}
One recent finding in the field is about knowledge leakage between train and evaluation sets~\cite{lewis2020question,emami2020analysis}. 
Similar concerns have motivated our careful training/evaluation splits (\S\ref{sec:experiments}) and experiments with varying training set sizes. 
Nevertheless, we found it challenging to define (and assess) the amount of leakage from the training data to evaluation. 
We welcome such studies on \name{}. 


\paragraph{Are we mimicking Google's QA?}
A reader might question the value of this work by noting that the website from which \name{} was mined had likely also used a QA system to begin with.
In other words, are we basically reverse-engineer Google's internal QA system~\changed{\cite{kilgarriff2007googleology}}?


% \ashish{Updated in various places:}
While we (the authors) are not aware of how Google answer box system works, we suspect that it is much more complex than a single QA system built using a single LM like T5~\cite{raffel2020exploring}. 
The system, besides incorporating one or more QA models, likely makes heavy use of implicit user feedback (e.g., information contained in billions of clicks, the structure of web links, etc.), in addition to explicit feedback from users and possibly some expert curation of answers to common questions.
Thus, the data in Google's answer boxes likely captures a variety of signals that contribute towards its high-quality. We believe aiming for a `standard' NLP QA system that's on par with Google QA is therefore a challenging and worthwhile goal.

\paragraph{Replicating human evaluation.}
One challenge with respect to the progress on the long-form QA task is the evaluation of responses. 
To facilitate future work on \name{} and replicability of our human evaluations, we have released the templates we have used to crowdsource human judgements.  
% are planning to provide evaluation API for human evaluation of model submissions, similar to the work of \citet{zellers2020evaluating}.  
There are also active proposals for streamlining the evaluation of text generation tasks~\cite{khashabi2021genie} which we might adopt.


\paragraph{Scope of our conclusions.}
It is worth emphasizing that one must be careful in taking these conclusions out of the context of this study (i.e., the dataset at hand, the models, the evaluation metrics used, etc.). 
While we hypothesize that these findings are relatively general, it might be possible to come up with a different long-form QA dataset on which the same baselines show a wildly different behavior.  


% \paragraph{Future work}
\paragraph{Other uses of \name{}.}
While we used \name{} for the purpose of QA, 
we hypothesize that this data with have a variety of use-cases: \emph{knowledge-base} accessible via questions queries~\cite{bosselut2019comet}, better question generation, etc. We leave such investigations for future work. 


% Given the breadth of \name{}, one can think of this as a \emph{knowledge-base} that is accessible through natural language queries~\cite{sap2019atomic,bosselut2019comet}. 
% % One other potential use-case for \name{} is using it as a \emph{knowledge-base} that is accessible through natural-language queries, similar to recent parallel efforts~\cite{sap2019atomic}. 
% Such a knowledge-base could be applicable to systems that work in interaction with knowledge-intensive modules~\cite{khot2020text}. \daniel{phrase it better?} 



==> UNUSED/intro-Hanna.tex <==
\section{Introduction}
% \daniel{Sewon: High-level comment: I think you are highlighting diverse types of answers, but it would be more interesting to highlight the *intrinsic* diversity of the task. I think the experiments already show that, but it was just not explicitly highlighted in the abstract/intro.}

Research in ``open'' question answering (also referred to as open-response, open-domain, or direct answer QA) has resulted in numerous datasets and powerful models for answering questions without a specified context. This task requires the use of background knowledge either stored in the QA model or retrieved from large corpora or knowledge bases~\cite{roberts2020much,lewis2020question}.
% \daniel{Edan: long sentence; drop it after "questions". }
% \tushar{Some cites introducing these prior research ideas would be helpful}. 
% The community, however, has focused mainly on short responses, with a few separate efforts on long response questions.
Existing effort, however, involves isolated studies on niche answer types, mainly short responses and, in a few cases, long responses~\cite{joshi2017triviaqa,lee2019latent,bhakthavatsalam2021think}.

In contrast, many of the everyday questions that humans deal with and pose to search engines have a more diverse set of response types, as illustrated in Fig.~\ref{fig:examples}. Their answer can be a multi-sentence description (a \emph{snippet}) (e.g., `what is' or `can you' questions), a \emph{collection} of items such as ingredients (`what are kinds of', `things to') or of steps towards a goal such as unlocking a phone (`how to'), etc. Even when the answer is short, it can have rich types, e.g., unit conversion, time zone conversion, or a variety of knowledge look-up (`how much', `when is', etc.).\footnote{In contrast, the short responses in existing datasets typically inquire about people, dates, and counts. For instance, 65\% of Natural Questions~\cite{kwiatkowski2019natural} begin with `who', `when', or `how many'; cf.~Fig~\ref{fig:bigram:distributions}.} Such answer type diversity is not represented in any existing dataset. 

Motivated by this, we introduce \name\ (pronounced \textit{guac}), the first open QA benchmark containing \emph{questions with all of the above answer types within a unified dataset, collected using the same, coherent process}. \name\ contains $3$ million questions with short, snippet, or collection answers, such as the ones shown in Fig.~\ref{fig:examples}.
Besides supporting research on various types of answers, \name\ enables a quantitative study of the inherent differences in systems across different answer types.

\name{} questions are automatically mined from Google's search-autocomplete feature and thus, we hypothesize, represent popular queries of real-world interest. Such questions also trigger `answer boxes' in the search results, containing responses deemed best by Google, which we extract and refer to as Google answers.
Our human evaluation of the dataset (\S\ref{subsec:data:quality}) found the collected questions and answers to be of high quality (about 94\%valid answers). 

\name\ provides a unified test bed to study inherent differences between questions. To do so, we fine-tune generative pre-trained language models (LM)~\cite{lewis2020bart,raffel2020exploring} on different subsets of \name, and ask whether models trained for different answer types:
%
\begin{enumerate}[noitemsep, label=(\subscript{Q}{{\arabic*}}),leftmargin=35pt]
    \item \label{q1} \emph{benefit similarly from pre-training?}
    \item \label{q2} \emph{benefit similarly from labeled data?}
    \item \label{q3} \emph{benefit similarly from larger models?}
\end{enumerate}






%We explore these questions in the context of generative pre-trained language models (LMs)~\cite{lewis2020bart,raffel2020exploring} as \emph{self-contained reasoners}, without explicit access to additional retrieved information. 

% \changed{by benchmarking} the powerful T5 language model~\cite{raffel2020exploring} on \name{} with both automatic metrics and human evaluation.
To understand the contribution of pre-training, {\bf \ref{q1}}, we train the powerful T5 language model~\cite{raffel2020exploring} on \name{}   with a small amount of labeled data. While LMs struggle, as expected, in this setting on \emph{short} response questions, they perform surprisingly well in generating \emph{snippet} and \emph{collection} responses \ashish{quantify `surprisingly well' by giving one sample number}\daniel{I am actually not sure how to do it so that its not misleading.}.
We hypothesize this is because response fluency and coherence have a much higher weight in such questions, and these factors remarkably benefit from the LM pre-training objective. 
%
Regarding the value of labelled data, {\bf \ref{q2}}, we observe the opposite trend: \emph{short} response questions benefit consistently from increasing amounts of supervised (labeled) data, whereas both \emph{snippet} and \emph{collection} response questions show minimal gains \ashish{again, quantify what minimal is}.
%
Lastly, on the benefit of model size, {\bf \ref{q3}}, we find larger models to be more effective in all cases as expected, but the gains are much more pronounced for \emph{snippet} and \emph{collection} response generation (20+\%) as compared to \emph{short} responses (5-10\%), under human evaluation. 

Additionally, we expect \name{} to facilitate further research on models for answering snippet and collection response questions.  While the largest models we consider score surprisingly high on these questions, they still lag behind 
% gold responses 
the upper-bound \ashish{are we referring to Google answers here or human performance?}
in both automated and human evaluations. Importantly, due to little benefit observed from more labeled data on such questions, further progress requires rethinking the solution approach.

Lastly, we find \name{} to be a valuable resource for training models. On the long-answer dataset ELI5~\cite{fan2019eli5}, T5 trained only on our snippet questions performs on par with state-of-the-art models trained on ELI5 data.

\changed{
Our closing remarks describe why we aren't simply replicating an existing QA system at Google, place our findings in context, and discuss future uses of \name{}, such as creating a neural knowledge-base or a question generation system. 
}

\paragraph{Contributions.} 
(a) We present \name, a collection of 3 million question-answer pairs with a diverse set of answers, along with a crowdsourced assessment of its quality.
(b) We benchmark state-of-art models on \name{}, both in terms of automatic and human judgments, and observe remarkable differences in how models behave w.r.t.\ various response types. 
(c) We demonstrate that \name{} is also a valuable model training resource by showing strong 
% zero-shot 
generalization to ELI5~\cite{fan2019eli5}. 
We hope this datatset will spur further research into open QA under diverse response types. 


==> UNUSED/intro-OLD.tex <==

%%% OLD ABSTRACT TEXT

\begin{comment}
% Google answers is pretty good which relies on user feedback
% How far is our SOTA open-domain QA technology?
In recent years, Google has added features that provide instant answers to many questions. 
% While little is known about the details of such platforms, we conjecture that the majority of Google's QA capabilities are enabled by techniques other than pure language understanding (e.g., through feedback from its users). 
In this work, we compare several state-of-the-art open-domain question-answering (QA) systems with Google's answers. 
The comparison is done on \name, a large-scale dataset with over 3 million questions/answers collected from Google.
\name{} questions are collected semi-automatically from the Google search engine using its autocomplete feature. This results in naturalistic questions of practical interest that are nonetheless short and expressed using simple language.  
We mine Google's responses to our collected questions from the answer boxes in the search results, which yields a rich space of answers containing both textual answers (short and long) as well as more structured ones such as collections. 
For evaluation on this dataset, we rely on judgments of crowdworkers since the resulting answers can be hard and difficult to handle by automatic evaluation metrics.  
We make the following empirical observations: 
(1) Direct human evaluation of \name{} indicates its high quality as evidenced by XX\% accuracy across different question types. 
(2) Current state-of-the-art open-domain QA models, on the other hand, achieve an accuracy of only ZZ\%, significantly worse than Google's performance.  
We release \name{} to facilitate further research on improving open-domain QA.\footnote{Data \& code to be released upon publication.}
% We further demonstrate that Qoogle is an effective pre-training dataset, helping improve performance across YY well-established reading comprehension benchmarks by WW\% on average.
\end{comment}


%%% OLD TEXT

\begin{comment}
The literature has such a lot of activity and progress on open-domain QA~\cite{berant2013semantic,lin2020tradeoffs}, thanks to fast development of deep pre-trained natural language models~\cite{devlin:bert,liu2019roberta,raffel2020exploring}.
In particular, we study the \emph{closed-book} variant of open-domain QA where LMs serve both as \emph{knowledgeable} reasoners~\cite{roberts2020much,lewis2020question,lee2020language}. 


In a parallel thread, search engines like Google have gotten significantly good at providing direct answers to many questions. 
These platforms are able to use a large amount of click information to help them effectively map input queries to a massive collection of information in their index~\cite{brin1998anatomy,joachims2002optimizing,joachims2017accurately}. 
% Hence, their ability is not all due to their intelligent in ....
Undeniably, portions of Google QA system use the well-established NLP machinery such as language models~\cite{nayak2019understanding}, however, the extent of their reliance on pure language-understanding is not clear. 
\end{comment}

% What are the extent of abilities of generative pre-trained natural language models~\cite{lewis2020bart,raffel2020exploring} in serving as a self-contained knowledgeable QA systems ? 

% \daniel{change the framing in this paragraph: we we to assess the ability of LMs models in the context open-domain QA; Google just happens to be our source of questions/answers.}

% \hanna{I would avoid starting the intro with closed-book QA; that's a pretty arbitrary term defined by the T5 paper; }
% We study the \emph{closed-book} variant of open-domain QA where generative pre-trained natural language models~\cite{lewis2020bart,raffel2020exploring} serve both as \emph{knowledgeable} reasoners, without access to any additional explicit information retrieval mechanism. 


% a collection of $3$ million open-domain question-answers collected using Google, which contains a variety of answer types (\emph{short} answers, \emph{snippet} answers, \emph{collection}  answers).

% \ashish{Two shortcomings to point out: (a) short questions in existing datasets tend to be somewhat homogeneous and often entity-centric $\Rightarrow$ ours are richer, (b) people in real world often pose other kinds of questions, those whose answers are snippets or collections. we have the first dataset that includes all these answer types in a single, coherent dataset that's collected in a uniform way. this results in a unified benchmark that facilitates comparing model behavior across various question types. we use it to answer 3 questions: (rephrase them in terms of the 3 big types: short, snippet, collection)}

% Questions posed by human users, such as to search engines, span many different answer types of questions in real world applications and in natural settings (Fig.~\ref{fig:examples}), varying from short answers (knowledge look-up, unit conversion, etc.) to a variety of long answers (e.g., descriptive responses, collection of steps towards a goal, etc). Unlike the abundance of resources and studies in questions \emph{short}-answer responses, these diverse forms of questions are less studied in the literature, mainly due to the lack of a unified benchmark with diverse answer types.

% \hanna{diverse answer types; natural question/every-day? and bring examples for these diverse types (refer to figure1).}
% However,  human users pose many different types of questions in real world applications and in natural settings (Figure 1), varying from short answers \daniel{(example categories)} to long answers (e.g., collections, instructions). Unlike the abundance of resources and studies in questions short-answer responses, these diverse forms of questions are less studied in the literature, mainly due to the lack of a unified benchmark with diverse answer types.

% \tushar{I would move the introduction to GooAQ here and move the following para right before the "We study GooAQ" para; motivating with "This benchmark of diverse answers allows us to study open-domainQA and focus on understanding the inherent."}
% In this paper, we introduce a benchmark to study open-domain QA for diverse forms of questions and focus on


\textbf{============ OLD INTRO BELOW ===========}

% To facilitate understanding differences between short and long answer responses, we create \name{}, a collection of $3$ million open-domain question-answers collected using Google, which contains a variety of answer types (\emph{short} answers, \emph{snippet} answers, \emph{collection}  answers).

% \hanna{
% And then the rest of the intro as it was
% -------- 
% }

% \tushar{Maybe clarify that this "long" form is different than NQ's long answer. Even a footnote would do.}

\begin{comment}
We study the open-domain QA where generative pre-trained natural language models~\cite{lewis2020bart,raffel2020exploring} serve both as \emph{self-contained} 
% knowledgeable 
reasoners, without access to any additional explicit information retrieval mechanism. 
% In this work, we compare the ability of several state-of-art open-domain QA systems to that of Google. 
While the previous work has extensively studied this setting for \emph{short} responses~\cite{roberts2020much,lewis2020question,lee2020language,min2021neurips,lewis2021paq}, there is very little work on \emph{long}-form questions\tushar{Maybe clarify that this "long" form is different than NQ's long answer. Even a footnote would do.} and comparisons between them. \tushar{Can we say something about the value of a dataset with the different question types and thereby GooAQ here? Otherwise it seems the entire purpose of building GooAQ was just to answer the three questions. It would be better if we could phrase it as "a open-domain QA dataset with short and long answer is useful and necessary(maybe). And btw, it also enables us to study these three questions."}
Broadly we are interested in understanding the inherent differences between  \emph{long} and \emph{short} response questions.
% In particular, we are interested in addressing the following questions: 
% \emph{
% \begin{enumerate}[noitemsep, label= (\subscript{Q}{0})]
%     % \item LMs do equally well on them? 
%     % \item On \emph{long}-answer questions, do LMs perform as well as they do on \emph{short} responses?  
%     % \item What is the benefit more labeled data each of long and short response questions? 
%     \item \label{q0} inherently, how do \emph{long} and \emph{short} response questions differ from each other? 
% \end{enumerate}
% }
% Additionally, we want to understand whether such differences 
% between \emph{long} vs \emph{short} response questions, 
% result in different outcomes when training models on them. 
Specifically, whether, 
\emph{
\begin{enumerate}[noitemsep, label= (\subscript{Q}{{\arabic*}})]
    \item \label{q1} they benefit similarly from labeled data? 
    \item \label{q2} they benefit similarly from pre-training? 
    \item \label{q3} they benefit similarly from larger models?
\end{enumerate}
}
\noindent
One of the main reasons why these questions have not yet been studied, we hypothesize, is because there is no single unified QA benchmark with diverse answer types. 


Towards this goal, we create \name{}, a collection of $3$ million open-domain question-answers collected using Google, which contains a variety of answer types (\emph{short} answers, \emph{snippet} answers, \emph{collection}  answers). 
\end{comment}
% answer boxes --- the portions of  the search result containing answers deemed the best to answer to the given query. 
% On the search engine results page, the answer box lists what Google deems is the best answer to the query. 
% It's positioned below the search query and above the organic results. 
% The quality of search engine features are heavily driven by the feedback received from their traffic.
% For example, search engines collect information about common questions, the pages that receive the most clicks and likely contain the answer the provided query. 
% , and hence, what snippets are likely to answer a given question.
% Hence, by creating a dataset from Google answer boxes, hat are the e are using the power of billions of clicks that are aggregated in the form of high-quality featured snippets. 

The questions in \name{} dataset are mined via search autocomplete which, we hypothesize, reflect a \emph{natural} distribution of the questions asked on Google.
% Inspired by earlier work~\cite{berant2013semantic,kwiatkowski2019natural} we use search auto-complete to collect commonly asked questions as they represent a more \emph{natural} distribution of the question.
Additionally, such questions due to their popularity tend to 
% also have the benefit that are more
% Prior to collecting any answer boxes, one has to compile a collection of questions that are most 
% likely to 
trigger answer boxes in the search results --- the portions of  the search result containing answers deemed the best to answer to the given query. 
% To mine such questions we use query auto-completion feature which reflects popular questions on Google's search platform. 


A key distinguishing feature of \name{}  is the diversity of its answers (see examples in Fig.~\ref{fig:examples}). 
For instance, {\color{darkgreen}`knowledge'} questions are typically about encyclopedic information (physics, history, etc.) typically with short responses. 
The {\color{darkgreen}`featured-snippet'} questions are the most popular in our collection which contain long multi-sentence answers. 
A subset of such questions also come with short responses. 
The answers to {\color{darkgreen}`collection'} questions are ordered or unordered set of phrases (for example, recipes, ingredients, steps) 
in response to goal posed in the question. 
% towards accomplishing a task.  
In addition to the diversity of answers, because the majority of the instances in \name{} have \emph{long} responses, 
% (e.g., `featured-snippet', `collection'), 
the dataset contains many `how'/`what' questions (\S\ref{subsec:statistics}) which are weakly covered by existing benchmarks and are less studied in the literature.  
\tushar{could we clarify which answer types are considered short and which are considered long answers? Or is that an orthogonal split?}\daniel{as per discussion with Ashish, we will better define what "long" means in the first two paragraph. Not changing this here until Ashish is done.}
% these questions (typically starting with `how' or `what') are among the less studied questions in the literature.  
% Additionally, we observe that \name{} contains questions (e.g., `how' questions) that are less mildly covered by the existing QA benchmarks. 
Such diversity of questions/answers make \name{} a valuable resource for better understanding the current state of open-domain QA across different classes of responses.

% Unlike the recent trends which is typically focus on building complex questions (input), here the questions use a relatively simple language and the majority of the complexity lies in the output space, e.g., answers that require explanation, comparison, listing steps, etc. 

\begin{comment}
For our purpose of comparing QA systems, it is important to have reliable way to evaluate the responses to input questions. 
Automatic metrics has worked reasonably well for the past for short response questions~\cite{lee2020language}. 
Since in our setup many questions demand relatively long responses, we also conduct crowd annotations (\S\ref{sec:experiments}), in addition to automatic evaluation.
% which makes the automatic evaluation less reliable. 
% direct-answer question could be a tricky, due to the richness of the answer responses. 
% In \name{}, the responses elicited from Google have a variety of forms. (explanations, collection, etc.) 
% For this reason, 
% \daniel{mention about empirical results here}
\end{comment}


% powered by the knowledge graph or scraped from a site that provides an adequate answer to a user's query.


% \hanna{
% experiment setup -- open QA,....
% Results
% why we think this benchmark and study useful. We showcase the benfit of our benchmark in long question answering in Eli5 in zero shot setting. We believe that our benchmark would facilitate .... and our study encourage reserach extension in diverse qas.
% }


We study \name{} as open-domain QA where generative pre-trained natural language models~\cite{lewis2020bart,raffel2020exploring} serve both as \emph{self-contained} 
% knowledgeable 
reasoners, without access to any additional explicit information retrieval mechanism. 
In particular, 
% We conduct a series of empirical work on \name{} . 
We benchmark T5~\cite{raffel2020exploring} a state-of-the-art model LM on \name{}, with both automatic metrics and human evaluation (\S\ref{sec:experiments}). 
% The results show that, on average, crowdworkers deemed \todo{x\%} of the responses as valid --- showing a reasonable quality for \name, in isolation from any other baseline. 
% Our results indicate that latest state-of-art models perform significantly inferior to Google, indicating that the platform is heavily reliant on technologies other than NLU.
% Our observations are multi-faceted: 
With respect to \ref{q1}, 
% evaluation of few-shot models indicate that, for 
we observe that pre-training carries most of the weight for \emph{long} response questions.  
% as models supervised with little labeled data have decent performance
% Consequently, 
% \tushar{actually I didn't get what does conversely imply here. pre-training harms it, doesn't help, doesn't help as much as labeled data?}
Empirically we observe that, even with \emph{little labeled data} the pre-trained models already have a decent performance in generating \emph{long} responses.However, that is not the case for \emph{short} response questions: LMs with little supervision are quite weak. 
We hypothesize this is because the response fluency and coherence have a much higher weight in \emph{long} response questions and these factors remarkably benefit from the existing pre-training objectives. 
% (as opposed to \emph{short} response questions in which factuality of the answers are dominant measure). 
% and to a lesser extent from pre-training
On \ref{q2}, we observe that \emph{short} response questions benefit much more from supervised (labeled) data: \emph{more} labeled data results in \emph{consistent gains}.  However, in \emph{long} response questions, our models show surprisingly \emph{minimal gains} when supervised with more labeled data. 
% We hypothesize that this is because short responses involve more factual responses, while in long 
On \ref{q3} we observe the trend of the past few years: larger models are better. 
However, the gains are much bigger for \emph{long} response generation. 

Overall, while our largest models achieve incredible heights in answering long response questions, they still perform worse than \name's gold responses.
Given that \emph{long} response questions benefit little from more annotated data, human parity performance requires rethinking our progress towards better models. 
We believe that \name{} will facilitate the field's progress towards addressing long-range open-domain questions.

% why we think this benchmark and study useful. We showcase the benfit of our benchmark in long question answering in Eli5 in zero shot setting. We believe that our benchmark would facilitate .... and our study encourage reserach extension in diverse qas.

\paragraph{Contributions.} 
(a) We present \name, a collection of 3 million question-answers pairs with a diverse set of answers. 
We conduct a series of crowdsorucing experiments which indicate a reasonable quality for our dataset. 
% indicate a high-quality quality for this dataset. 
% \tushar{Maybe there is a better phrasing for this, but currently it reads like what }
% The results show that, on average, crowdworkers deemed \todo{x\%} of the responses as valid --- showing a reasonable quality for \name, in isolation from any other baseline. 
% We show the quality of the responses the feedback of crowdworkers. 
% (c) We show the value pre-training on \name.
(b) We benchmark state-of-art models on \name{}, both in terms of automatic and human judgments, and observe differences in how various question types are treated by these models. 
(c) We showcase the benefit of our collected data in answering long answers, by conducting zero-shot generalization to ELI5~\cite{fan2019eli5}. 
% another long-form QA dataset collected from Reddit.
% \hanna{somewhere, we need to invite researchers in the field to use our collected data?}
We hope this datatset will be bring more light to the study of QA under diverse types. 



\begin{comment}
We show that pre-training on \name{} benefits the performance across \todo{xx} well-established datasets. 
Additionally, we create a generative QA task based on our collected dataset and pose it as a challenge for the field. 
We train several-state-of-art models for this task and show that 



\paragraph{Contributions.} (a) we present \name, a collection of 3 million question-answers pairs with a diverse set of answers, and 
(b) show that it's reasonably quality through crowdsourcing experimets.  
% We show the quality of the responses the feedback of crowdworkers. 
% (c) We show the value pre-training on \name. 
(c) We frame a challenge task based on our collected data, and
% We create challenge tasks based on our dataset and show empirically show that state-of-art models struggle on this task.  
(d) empirically show that latest state-of-art models struggle on this task.  
\end{comment}




==> UNUSED/intro-OLD2.tex <==
\section{Introduction}

Research in ``open'' question answering (also referred to as open-response, open-domain, or direct answer QA) has resulted in numerous datasets and powerful models for answering questions without a specified context, by using background knowledge either stored in the QA model or retrieved from large corpora or knowledge bases~\cite{roberts2020much,lewis2020question}
% \tushar{Some cites introducing these prior research ideas would be helpful}. 
\changed{
% The community, however, has focused mainly on short responses, with a few separate efforts on long response questions.
There are, however, a series of isolated studies on niche answer types, mainly on short responses a few separate efforts on long response questions~\cite{ joshi2017triviaqa,lee2019latent,bhakthavatsalam2021think}
}

In contrast, many of the everyday questions that humans deal with and pose to search engines have a more diverse set of response types, as illustrated in Fig.~\ref{fig:examples}. Their answer can be a multi-sentence description (a \emph{snippet}) (e.g., `what is' or `can you' questions), a \emph{collection} of items such as ingredients (`what are kinds of', `things to') or of steps towards a goal such as unlocking a phone (`how to'), etc. Even when the answer is short, it can have richer types, e.g., unit conversion, time zone conversion, or various kinds of knowledge look-up (`how much', `when is', etc.).\footnote{In contrast, the short responses in existing datasets typically inquire about people, dates, and counts (e.g., 65\% of Natural Questions~\cite{kwiatkowski2019natural} begin with `who', `when', or `how many'; cf.~Fig~\ref{fig:bigram:distributions}).} Such answer type diversity is not represented in any existing dataset. 

Motivated by this, we introduce \name\ (pronounced \textit{guac}), the first open QA benchmark containing \emph{questions with all of the above answer types within a unified dataset, collected using the same, coherent process.} 
\changed{
Besides supporting research on various types of answers, \name\ enables a quantitative study of the inherent differences in systems across different answer types. Specifically, we use \name{} to ask whether models for different answer types:
}
%
\begin{enumerate}[noitemsep, label=(\subscript{Q}{{\arabic*}}),leftmargin=35pt]
    \item \label{q1} \emph{benefit similarly from pre-training?}
    \item \label{q2} \emph{benefit similarly from labeled data?}
    \item \label{q3} \emph{benefit similarly from larger models?}
\end{enumerate}


\begin{comment}
===================

Research in ``open'' question answering (also referred to as open-response, open-domain, or direct answer QA) has resulted in numerous datasets and powerful models for answering questions without a specified context, by using background knowledge either stored in the QA model or retrieved from large corpora or knowledge bases\tushar{Some cites introducing these prior research ideas would be helpful}.  Open QA datasets, however, focus mainly on short responses~\cite{berant2013semantic,joshi2017triviaqa,lee2019latent,lewis2021paq,bhakthavatsalam2021think},
% and subsequently, powerful pre-trained language models (LM) supervised with such datasets
% for building models and analysis of  to \emph{short} response QA datasets
and so do the models designed for them~\cite{roberts2020much,lewis2020question,lee2020language,min2021neurips,lewis2021paq}. Further, the short responses considered typically inquire about people, dates, and counts (e.g., 65\% of Natural Questions~\cite{kwiatkowski2019natural} begin with `who', `when', or `how many'; cf.~Fig~\ref{fig:bigram:distributions}). 

In contrast, many of the everyday questions that humans deal with and pose to search engines have a more diverse set of responses, as illustrated in Fig.~\ref{fig:examples}. Their answer can be a multi-sentence description (a \emph{snippet}) (e.g., `what is' or `can you' questions), a \emph{collection} of items such as ingredients (`what are kinds of', `things to') or of steps towards a goal such as unlocking a phone (`how to'), etc. Even when the answer is short, it can have richer types, e.g., unit conversion, time zone conversion, or various kinds of knowledge look-up (`how much', `when is', etc.). Such answer type diversity is not represented in any existing dataset. 

% \hanna{how about adding an opening paragraph like this}
% \hanna{In this paper,  we introduce \name, the first open QA benchmark containing questions with all of the above answer types within a unified dataset, collected using the same, coherent process. Moreover, we evaluate efficacy of  pretrained language models in answering these questions and collectively study their inherent differences using \name. }

We 
% propose 
\changed{introduce}
\name\ (pronounced \textit{guac}), the first open QA benchmark containing \emph{questions with all of the above answer types within a unified dataset, collected using the same, coherent process.} 
\changed{
% On this dataset, we evaluate efficacy of pre-trained LMs and study their behavior on various answer types.  
We use this dataset to evaluate the efficacy and the behavior of pre-trained LMs on these various answer types.
}
\hanna{how about this? We use this dataset to support research in answering questions with various answer types, particulary in evaluating the efficacy and the behavior of pre-trained LMs on these questions.}
\hanna{or this? We use this dataset in evaluating the efficacy and the behavior of pre-trained LMs on these various answer types, supporting research in answering diverse types of questions .}

\end{comment}

% Specifically, 
\name{} contains $3$ million questions with short, snippet, or collection answers, such as the ones shown in Fig.~\ref{fig:examples}. \ashish{TODO: include some noteworthy X\% stats}. \name{} questions are automatically mined from Google's search-autocomplete feature and thus, we hypothesize, represent popular queries of real-world interest. Such questions also trigger `answer boxes' in the search results, containing responses deemed best by Google, which we extract and use as the gold answer.

% \daniel{Hanna: until these questions it seems that we're reading a dataset paper.}

\begin{comment}
Having a variety of answer types within a single, coherent, open QA benchmark enables a quantitative study of the inherent differences across them. Specifically, we use \name{} to ask whether models for different answer types:
%
\begin{enumerate}[noitemsep, label=(\subscript{Q}{{\arabic*}}),leftmargin=35pt]
    \item \label{q1} \emph{benefit similarly from pre-training?}
    \item \label{q2} \emph{benefit similarly from labeled data?}
    \item \label{q3} \emph{benefit similarly from larger models?}
\end{enumerate}
\end{comment}


We explore these questions in the context of generative pre-trained language models (LMs)~\cite{lewis2020bart,raffel2020exploring} as \emph{self-contained reasoners}, without explicit access to additional retrieved information. 
In particular, we benchmark the powerful T5 language model~\cite{raffel2020exploring} on \name{}, with both automatic metrics and human evaluation (\S\ref{sec:experiments}). 

To study {\bf \ref{q1}}, we train models (separately for each response type) with a small amount of labeled data (2$k$ questions), mainly to convey the nature of the task. While LMs struggle, as expected, in this setting on \emph{short} response questions, they perform surprisingly well in generating \emph{snippet} and \emph{collection} responses (e.g., humans prefer T5-11B's response to Google's response in 30\% of such questions; Fig.~\ref{fig:eval}, bottom-right plots).
We hypothesize this is because response fluency and coherence have a much higher weight in such questions, and these factors remarkably benefit from the LM pre-training objective. 
On {\bf \ref{q2}}, we observe the opposite trend: \emph{short} response questions benefit consistently from increasing amounts of supervised (labeled) data, whereas both \emph{snippet} and \emph{collection} response questions show minimal gains. \tushar{Much longer explanation for Q1 than the other questions. I personally prefer these shorter summaries. We could probably gloss over many of the details in the explanation for Q1.}
On {\bf \ref{q3}}, larger models, as expected, are more effective in all cases, but the gains are much more pronounced for \emph{snippet} and \emph{collection} response generation (20+\%) as compared to \emph{short} responses (5-10\%), under human evaluation. 

We hope \name{} will facilitate research towards improving models to answer snippet and collection response questions.  While the largest models we consider score surprisingly high 
% achieve surprisingly high scores 
on these questions, they still lag behind 
% gold responses 
\changed{the upper-bound}
in both automated and human evaluations. Importantly, due to little benefit observed from more 
% annotated 
\changed{labeled}
data on such questions, \changed{further progress} 
% human parity 
requires rethinking our approaches. 
% approach towards better models.

We find \name{} to be a valuable resource for training models. 
\begin{comment}
E.g., T5 trained on our snippet questions shows strong
% zero-shot  
% \daniel{rephrase: with no training on the target data}
generalization to ELI5~\cite{fan2019eli5}, a long-answer dataset, achieving a score \changed{on-par} with
% within \daniel{X\%} of 
the state-of-the-art models trained using ELI5 data. 
\end{comment}
\changed{
% It's not obvious that your model was not trained on ELI5. Maybe "
On the long-answer dataset ELI5~\cite{fan2019eli5}, T5 trained only on our snippet questions performs on-par with the state-of-the-art models trained on ELI5 data.}

\paragraph{Contributions.} 
(a) We present \name, a collection of 3 million question-answer pairs with a diverse set of answers, along with a crowdsourced assessment of its quality.
(b) We benchmark state-of-art models on \name{}, both in terms of automatic and human judgments, and observe remarkable differences in how models behave w.r.t.\ various response types. 
(c) We demonstrate that \name{} is also a valuable model training resource by showing strong 
% zero-shot 
generalization to ELI5~\cite{fan2019eli5}. 
We hope this datatset will spur further research into open QA under diverse response types. 


==> UNUSED/obsolete.tex <==

\begin{comment}
 The availability of rich datasets remains to be a bottleneck for building and evaluating stronger NLP systems. 
%  Having large-scale dataset for supervising QA is still valuable. 
%  large-scale 
%  distantly-supervised 
%  rich answer space
 In this work, we introduce \name{}, a large-scale dataset of  question-answers, semi-automatically mined from Google. 
 The mined questions, while having a relatively simple language, cover a wide range of questions that are common among Google users. 
 The mined answers span a rich space of responses: short answer, long answer, collection, etc --- a major deviations from many existing popular datasets. 
 We show that pre-training on \name{} helps improve performance across \todo{x} well-established reading-comprehension datasets. 
 Additionally, we define challenge tasks based on our collected questions. 
 We build baselines for the proposed challenge and, based on human evaluation of the results, we show the difficulty of the task for the current state-of-the-art models.\footnote{Data \& code to be released upon publication.}
\end{comment}


% Nov 20 
In order to help build and evaluate stronger NLP systems, we introduce \name, a large scale question-answering (QA) dataset with over 3 million questions and with a rich answer space.
\name{} questions are collected semi-automatically from the Google search engine using its auto-complete feature. This results in naturalistic questions of practical interest that are nonetheless short and expressed using simple language.  
Furthermore, answers to \name{} questions are mined from the answer-boxes in the search results, which yields a rich space of answers containing both textual answers (short and long) as well as more structured ones such as collections. 
Despite its semi-automatic construction, \name{} represents a high quality dataset as evidenced by over XX\% accuracy in our human evaluation. Current state-of-the-art models, on the other hand, achieve an accuracy of only ZZ\%, setting \name{} up as a challenging QA benchmark for the academic community.\footnote{Data \& code to be released upon publication. 



\section{Related work}
We review several related lines of work. 
\paragraph{Search engines as a source of supervision.}
There several prior work that have used search engines for 
% We are not the first to use search results to for 
collecting resources for AI systems. 
Search engines are able to use a large amount of click information to help them effectively map input queries to a massive collection of information in their index~\cite{brin1998anatomy,joachims2002optimizing,joachims2017accurately}. 
% Hence, their ability is not all due to their intelligent in ....
Although academic researcher do not have direct access to click information, rankings of search engines are a valuable source information that allow for indirect supervision. 
For instance, in the computer vision literature, image search is often used to harness signals for tasks like building object detection or classifications~\cite{fergus2005learning,fernando2013mining,chen2015webly}. 
Similarly, it the context of NLP applications it has been used for tasks like entity recognition~\cite{rud2011piggyback} or pronoun resolution~\cite{peng2015solving}. 


\paragraph{Large QA datasets.}
% including mining QA datasets.
The recent literature has seen an increase in publication of large-scale QA datasets. 
Several of such datasets are collected with the help of crowdworkers~\cite{rajpurkar2016squad,trischler2017newsqa,kovcisky2018narrativeqa}. 

%% talk about the diversity of the answers 
Among the recent datasets a consistent trend is about building datasets with more complex questions. 
For example, 
unanswerable questions~\cite{rajpurkar2018know}, 
multi-sentence questions~\cite{khashabi2018looking}, 
quantitative-reasoning questions~\cite{dua2019drop}, inter alia. 
Unlike such works, our questions (inputs) come with relatively  simple phrasing, as they are samples of natural queries. 
However, the majority of the complexity lies is in the output space: short answers for different questions types, long explanation-like responses, collections (recipes, ingredients, etc).  
% While there has been a consistent progress towards building dataset with rich \emph{input} questions, the richness of the output space is rarely the topic of the study. 


There are several datasets that, at least partially, rely on mining their questions/answers. Several notable such datasets are listed in Table~\ref{fig:comparison:table} \cite{berant2013semantic,hermann2015teaching,nguyen2016ms,joshi2017triviaqa,kwiatkowski2019natural}. 
For instance, WebQuestions~\cite{berant2013semantic} uses search auto-complete API for collecting their questions, like \name. However, they use crowdsourcing to annotate the answers to these questions. 
NaturalQuestions contains queries issued to Google and crowdsource long and short answers for each questions. 
\daniel{cite the OD variant of NQ and TriviaQA}
Our questions are similar to that of NaturalQuestions, however, our data contains more instances and a more diverse types of answers.
Among the listed set, CNN/DailyMail is the largest dataset constructed with an automated process based on paragraph summaries mined news websites. Our presented dataset does not use any rule-based constructions for its building and it is several orders of magnitude larger than CNN/DailyMail. 
    
% SQuAD~\cite{rajpurkar2016squad,rajpurkar2018know}
% The Stanford Question Answering Dataset (SQuAD) is a dataset designed for reading comprehension tasks. Crowd workers are employed to ask questions over a set of Wikipedia articles. They are then asked to annotate the questions with the text segment from the article that forms the answer. In a second version, they add ca. 50,000 unanswerable questions to the dataset. These questions, too, are generated by crowd workers over Wikipedia articles.


% WebQuestions~\cite{berant2013semantic}
%  Berant et al. use the Google Suggest API as basis for generating questions. They start with a single question ("Where was Barack Obama born") and feed the Google Suggest API with three query fragments generated from the source question: the question without the phrase before the entity, the question without the entity and the question without the phrase after the entity. Each of these queries generates 5 candidate questions. The candidate questions are added to a queue of questions and the process is repeated for each of the questions in the queue. They stop after 1M questions are generated. Due to the nature of the approach, the generated questions start with a wh-word and revolve around a single entity. 100K of these questions are given to crowdsourcing workers who select a Freebase entity, value or list of entities as answer. Questions that are answered identically by at least two workers are included in the dataset.


% CNN/DailyMail~\cite{hermann2015teaching}
% Hermann et al. construct a reading comprehension dataset by collecting articles from the CNN and DailyMail websites. They use the websites' summarization statements to create Cloze style questions by replacing single entities with placeholders. Entities are anonymized within articles to prevent systems from infering answers using general world knowledge.

% Children's Book Test (CBT)~\cite{hill2015goldilocks}
% Hill et al. construct a reading comprehension dataset from 108 children's books. An example consists of context, query, answer candidates and the actual answer. The context consists of 20 consecutive sentences. A single word is removed from the 21st sentence such that the sentence forms the query and the removed word forms the answer. The answer candidates consist of 9 words that appear within the 21 sentences and have the same type as the answer (named entity, common noun, verb, preposition) plus the actual answer.

% 30M Factoid Question-Answer Corpus~\cite{serban2016generating}
% Serban et al. use an encoder-decoder architecture to generate questions from Freebase facts (subject - predicate - object triples). Their system is trained on the SimpleQuestions dataset by Bordes et al. .


% TriviaQA~\cite{joshi2017triviaqa}, etc.
% Joshi et al. collect question-answer pairs from 14 trivia websites. Additionally, they gather textual evidence for the given answer from Web Search results and Wikipedia articles.


% MS MARCO~\cite{nguyen2016ms}
% The MS MARCO dataset contains search queries submitted via Bing or Cortana. For each query, the dataset contains text passages from documents that are provided by Bing as a result for the given query. 182,669 queries additionally come with answers generated by crowd workers.


% ComQA~\cite{abujabal2019comqa}
% Abujabal et al. extract questions from the WikiAnswers website. The questions are grouped into paraphrase clusters using crowd-sourcing.

% NQ~\cite{kwiatkowski2019natural}, 
% The questions come from real queries issued to the Google search engine. Human annotators were given the question together with a Wikipedia page from the top-5 search results, and marked a long answer (a paragraph) and a short answer (the target span) in the article, or null if the answer was not present in the article. Questions were excluded if the annotators classified them as ambigous, incomprehensible, dependent on clear false presuppositions, opinion-seeking, or not clearly a request for factual information.

% WikiSuggest~\cite{choi2017coarse}
% the data does not seem to be available 
% on a new dataset called WIKISUGGEST that contains more natural questions gathered from a search engine
% We use the Google Suggest API to harvest natural language questions and submit them to Google Search. Whenever Google Search returns a box with a short answer from Wikipedia (Figure 3), we create an example from the question, answer, and the Wikipedia document.



